Higher-Order Cheeger Inequality for Partitioning with Buffers

We prove a new generalization of the higher-order Cheeger inequality for partitioning with buffers. Consider a graph $G=(V,E)$. The buffered expansion of a set $S \subseteq V$ with a buffer $B \subseteq V \setminus S$ is the edge expansion of $S$ after removing all the edges from set $S$ to its buffer $B$. An $\varepsilon$-buffered $k$-partitioning is a partitioning of a graph into disjoint components $P_i$ and buffers $B_i$, in which the size of buffer $B_i$ for $P_i$ is small relative to the size of $P_i$: $|B_i| \le \varepsilon |P_i|$. The buffered expansion of a buffered partition is the maximum of buffered expansions of the $k$ sets $P_i$ with buffers $B_i$. Let $h^{k,\varepsilon}_G$ be the buffered expansion of the optimal $\varepsilon$-buffered $k$-partitioning, then for every $\delta>0$, $$h_G^{k,\varepsilon} \le O_\delta(1) \cdot \Big( \frac{\log k}{ \varepsilon}\Big) \cdot \lambda_{\lfloor (1+\delta) k\rfloor},$$ where $\lambda_{\lfloor (1+\delta)k\rfloor}$ is the $\lfloor (1+\delta)k\rfloor$-th smallest eigenvalue of the normalized Laplacian of $G$. Our inequality is constructive and avoids the ``square-root loss'' that is present in the standard Cheeger inequalities (even for $k=2$). We also provide a complementary lower bound, and a novel generalization to the setting with arbitrary vertex weights and edge costs. Moreover our result implies and generalizes the standard higher-order Cheeger inequalities and another recent Cheeger-type inequality by Kwok, Lau, and Lee (2017) involving robust vertex expansion.

==> sections/background.tex <==
\section{Introduction}



\section{Background}
In this note\footnote{Kostya: The first section is based on my old notes about Cheeger's inequality. I slightly reworked them.}, we prove Cheeger's inequality for regular expanders. Let $G = (V,E)$ be a $d$-regular
expander on $n$ vertices. The two key
parameters of the expander $G$ are the edge expansion $h_G$ and
the second eigenvalue of the Laplacian $\lambda_G$. The edge expansion
gives a lower bound on the size of every cut: for every subset of vertices
$S\subset V$, the size of the cut between $S$ and $|V\setminus S|$ is at least
$$h_G \times \frac{\min (|S|, |V\setminus S|)}{|V|} |E|.$$
It is formally defined as follows:
$$h_G =
\min_{S \subset V}
\left(\frac{|\delta(S,V\setminus S)|}{|E|} \left/
\frac{\min (|S|, |V\setminus S|)}{|V|}\right. \right),$$
here $\delta(S,V\setminus S)$ denotes the cut --- the set of edges going from $S$ to $V\setminus
S$. The Laplacian $L_G$ of the graph $G$ is defined as
\begin{equation}\label{eq:lapl}
\langle v,L_Gv\rangle = \frac{1}{d}\sum_{(i,j)\in E} (v(i) - v(j))^2.
\end{equation}
Its matrix representation is as follows
$$L_G(i,j)  =
\begin{cases}
1, & \text{if } i=j\\
-1/d, & \text{if } (i,j) \in E\\
0, &\text{otherwise.}
\end{cases}
$$
%%The smallest eigenvalue of $L_G$ is 0; and the corresponding eigenvector is a vector of all 1's,
%%denoted by~$\ONE$. Thus
%%$$\lambda_G = \min_{x \perp \text{\large{\textbf{1}}}} \frac{\iprod{x}{L_Gx}}{\|x\|^2}.$$
%%Cheeger's inequality,
%%$$h_G^2/8 \leq \lambda_G \leq h_G,$$
%%shows that $h_G$ and $\lambda_G$ are closely related; however $\lambda_G$ can be much smaller than $h_G$
%%(the lower bound
%%in the inequality is tight).

The smallest eigenvalue of $L_G$ is 0; and the corresponding eigenvector is a
vector of all 1's, denoted by~\large{\textbf{1}}. The second eigenvalue, denoted by
$\lambda_G$, is in a sense a continuous analog of the edge expansion. It turns out
that
$$h_G^2/8 \leq \lambda_G \leq h_G.$$
This inequality is known as Cheeger's inequality. In this note, we shall prove this inequality.

We first prove the ``easy part'' of Cheeger's inequality: $\lambda_G \leq h_G$. We start with the following
observation about the connection between cuts in the graph and the Laplacian operator.
\begin{observation}\label{obs:cut-size-L}
Let $S$ be a subset of vertices $G$; and let $v$ be its ``indicator'' vector:
$$v(i) = \begin{cases} 1,& \text{if } i \in S;\\0,& \text{otherwise }.\end{cases}$$
Then
$$\langle v, L_G v\rangle = \frac{\delta(S,V\setminus S)}{d}.$$
\end{observation}
\begin{proof}
Follows from~(\ref{eq:lapl}).
\end{proof}

Another basic observation we need is that
\begin{equation}\label{eq:minform}
\lambda_G = \min_{x \perp \ONE} \frac{\langle x,L_G x\rangle}{\|x\|^2},
\end{equation}
this trivially follows from the fact that $\ONE$ is the eigenvector corresponding to the
eigenvalue 0; and that $L_G$ is a self-adjoint operator, or, in other words, the matrix $L_G$ is symmetric.

Pick the sparsest cut $S$ and consider its indicator vector $v$. We represent $v$ as a sum of two perpendicular vectors
$v = \VOne +  \VPerp$, where the first vector $\VOne$ is
collinear with the vector \large{\textbf{1}}; and the second vector $\VPerp$ is orthogonal to \large{\textbf{1}}.
Since $\VPerp \perp \ONE$, we have by (\ref{eq:minform}),
$$\lambda_G = \min_{x \perp \ONE} \frac{\langle x,L_G x\rangle}{\|x\|^2}
\leq \frac{\langle \VPerp, L_G \VPerp\rangle}{\| \VPerp\|^2}.$$
Using Observation~\ref{obs:cut-size-L}, write
$$
\frac{\delta(S,V\setminus S)}{d} = \langle v, L_G v \rangle = 
\langle (\VPerp + \VOne), L_G (\VPerp + \VOne) \rangle
= \langle \VPerp, L_G \VPerp\rangle.$$
Here, we used that $L_G \VOne = 0$. Vector 
$\VOne$ is the projection of $v$ onto the unit vector 
$\ONE/\|\ONE\|$. Thus, 
$$\VOne = 
\big\langle\frac{\ONE}{\|\ONE\|}, v\big\rangle \cdot \frac{\ONE}{\|\ONE\|} = 
\frac{\langle\ONE, v\rangle}{\|\ONE\|^2} \cdot \ONE;
\text{ and } \VPerp = v - \VOne = v - \frac{\langle\ONE, v\rangle}{\|\ONE\|^2}
\ONE.$$
Consequently,
$$
\|\VPerp\|^2 = \left\|v - \frac{\langle\ONE, v\rangle}{\|\ONE\|^2}
\ONE\right\|^2= |S| \times \left(1-\frac{|S|}{n}\right)^2 + (n-|S|) \times \left(-\frac{|S|}{n}\right)^2 =
\frac{|S|\times |V \setminus S|}{n}.$$
Thus
$$\lambda_G \leq \frac{\langle \VPerp, L_G \VPerp\rangle}{\| \VPerp\|^2} = 
\frac{\delta(S,V\setminus S)}{d|S|\times (|V\setminus S|/n)}
\leq
\frac{2\delta(S,V\setminus S)}{d|S|}.$$
The right hand side of this inequality is the edge expansion of the graph:
$$h_G = \frac{\delta(S, V\setminus S)}{dn/2} \left/  \frac{|S|}{n}  \right. = \frac{2\delta(S, V\setminus S)}{d |S|}.$$
This completes the proof of the ``easy'' part of Cheeger's inequality. 

We now prove the ``hard'' part of the inequality: $h_G^2/8\leq \lambda_G$. To this end, we show how to find a random cut $S$ in the graph $G$
using the second eigenvector of $L_G$. Note that for every distribution of sets $S$ of size at most $n/2$, we have (prove it!) 
$$h_G \leq \frac{\E|\delta(S,V\setminus S)|}{|E|} \left/
\frac{\E|S|}{|V|} = \frac{\E|\delta(S,V\setminus S)|}{\E|S|} \cdot \frac{|V|}{|E|}\right.
= \frac{2}{d}\cdot \frac{\E|\delta(S,V\setminus S)|}{\E|S|}.
$$
So, our goal is to define a probability distribution of cuts $S$ with $\E|\delta(S,V\setminus S)|/\E|S|\leq d\sqrt{2\lambda_G}$

Let $v$ be an eigenvector
of $L_G$ corresponding to $\lambda_G$. Then, $v \perp \ONE$, in other words $v(1)+v(2)+\dots+v(n)=0$ and
\begin{equation}\label{eq:v-LG-v-bound}
\langle v, L_G v\rangle = \lambda_G \|v\|^2.    
\end{equation} 
For technical reasons, we need to split vector $v$ into two vectors $v_+$ and $v_-$ each having at most $n/2$ non-zero coordinates. We do this as follows. First, we sort the vertices of the graph in decreasing order i.e. we assume that $v(1)\geq v(2) \geq \dots \geq v(n)$. Denote $m=\roundup{n/2}$; and
$\mu = v(m)$. Then, $\mu$ is the median of $v(1),\cdots, v(n)$. Define $v_+$ and $v_-$ as follows:
$$v_+ (i)= \begin{cases}
v(i) -\mu,& \text{if } i \leq m;\\
0,& \text{otherwise}.
\end{cases}
$$

$$v_- (i)= \begin{cases}
0,& \text{if } i \leq m;\\
v(i)-\mu,& \text{otherwise}.
\end{cases}
$$
We will show that at least one of the following inequalities holds: $\langle v_+, L_G v_+\rangle \leq \lambda_G \|v_{+}\|^2$ or $\langle v_-, L_G v_-\rangle \leq \lambda_G \|v_{-}\|^2$. These inequalities are similar to the bound (\ref{eq:v-LG-v-bound}) we have for vector $v$. 

\begin{claim}\label{cl:v-plus-v-minus}
For vectors $v_+$ and $v_-$ defined above, we have 
\begin{enumerate}
    \item $\|v\|^2  \leq \|v_{+}\|^2 + \|v_{-}\|^2;$ and
    \item $\langle v, L_G v\rangle \geq\langle v_+, L_G v_+\rangle +  \langle v_-, L_G v_-\rangle$;
    \item $\langle v_+, L_G v_+\rangle \leq \lambda_G \|v_{+}\|^2$ or $\langle v_-, L_G v_-\rangle \leq \lambda_G \|v_{-}\|^2$.
\end{enumerate}
\end{claim}
\begin{proof}
First, we make several simple observations. Vectors $v_+$ and $v_-$ are orthogonal because their supports are disjoint. All coordinates of $v_+$ are non-negative, and all coordinates of
$v_-$ are non-positive. Finally, $v_{+} + v_{-} = v - \mu \ONE$. Thus, 
$$\|v_{+}\|^2 + \|v_{-}\|^2=  \|v_{+} + v_{-}\|^2
=\|v - \mu \ONE\|^2
=\|v\|^2 -\underbrace{2\mu \langle v, \ONE\rangle}_{=0} + \mu^2 \|\ONE\|^2 \geq \|v\|^2.
$$
This proves item (1). We now use that $\ONE \in \ker L_G$ i.e., $L_G\ONE = 0$. Write,
\begin{multline*}
\langle v, L_G v\rangle = \langle v - \mu\ONE, L_G(v-\mu\ONE)\rangle =
\\=
\langle v_+, L_G v_+\rangle +  \langle v_-, L_G v_-\rangle +  \underbrace{2\langle v_-, L_G v_+\rangle}_{\geq 0}
\geq \langle v_+, L_G v_+\rangle +  \langle v_-, L_G v_-\rangle.
\end{multline*}
The last inequality holds because all off diagonal entries in $L_G$ are non-positive;  $v_+(i)v_-(j)\leq 0$ for all $i,j$; and $v_+(i)v_-(i) = 0$. This proves item (2).

We have
$$\langle v_+, L_G v_+\rangle +  \langle v_-, L_G v_-\rangle \leq \langle v, L_G v\rangle =
\lambda_G \|v\|^2 \leq \lambda_G (\|v_{+}\|^2 + \|v_{-}\|^2).$$
Thus, $\langle v_+, L_G v_+\rangle \leq \lambda_G \|v_{+}\|^2$ or $\langle v_-, L_G v_-\rangle \leq \lambda_G \|v_{-}\|^2$.
\end{proof}

Without loss of generality assume that
\begin{equation}\label{eq:bound-v-plus}
\langle v_+, L_G v_+\rangle \leq \lambda_G \|v_{+}\|^2.
\end{equation}

We now show how to pick a set $S$ using a random threshold cut. We draw a random number $t$ in the range $(0,v_+(0)^2)$ (recall that $v_+(0)$ is the largest coordinate of $v_+$). Then, we set $S=\{i: v(i)^2 > t\}$.  Observe, that the size of $|S|$ is always less than $n/2$ as required, because $v_+$ has at most $n/2$ non-zero entries (remark: this is the reason why we split vector $v$ into two vectors, $v_+$ and $v_-$, with at most $n/2$ non-zero coordinates).

For the analysis of the algorithm, we assume that 
$v_+(1) = 1$. This can be done by scaling the vector $v$. Then, all coordinates of $v_+$ lie in the interval $[0,1]$. Our goal is to upper bound
$\E[\delta(S,V\setminus S)]/\E|S|$.

Let us first compute the expected size of $S$.  The probability that $i$ belongs to $S$ equals $v_+(i)^2$, thus
$$\E{|S|} = \sum_{i=1}^n |v_+(i)|^2 = \|v_+\|^2.$$
Then, we find an upper bound on the expected size of the cut
\begin{eqnarray}
\E{|\delta(S,V\setminus S)|} &=& \sum_{(i,j)\in E} |v_+(i)^2 - v_+(j)^2| = \sum_{(i,j)\in E} |v_+(i) - v_+(j)| \times |v_+(i) + v_+(j)|\\
&\leq&  \sqrt{\sum_{(i,j)\in E} |v_+(i) - v_+(j)|^2} \times \sqrt{\sum_{(i,j)\in E} |v_+(i) + v_+(j)|^2}.
\label{eq:exp-cut-size}
\end{eqnarray}
The first term on the right hand side equals 
$\sqrt{d\langle v_+, L_G v_+\rangle}$, which is at most $\sqrt{d\lambda_G} \|v_+\|$ by inequality  (\ref{eq:bound-v-plus}). Then,
$$\sum_{(i,j)\in E} |v_+(i) + v_+(j)|^2\leq
2\sum_{(i,j)\in E} v_+(i)^2 + v_+(j)^2
=
2d\sum_{(i,j)\in E} v_+(i)^2 = 2d \|v_+\|^2.
$$
Here, we used that the graph is $d$-regular, and thus every vertex appears in the second sum exactly $d$ times. We now plug this bound in~(\ref{eq:exp-cut-size}), and obtain the following bound on the expected cut size:
$$\E{|\delta(S,V\setminus S)|}
\leq \sqrt{\lambda_G d} \|v_+\|\times \sqrt{2d \|v_+\|^2} = \sqrt{2\lambda_G} \times d\|v_+\|^2.$$
We have 
$$\frac{\E{|\delta(S,V\setminus S)|}}{\E[|S|]}\leq
\frac{\sqrt{2\lambda_G} \times d\|v_+\|^2}{\|v_+\|^2} = d\cdot \sqrt{2\lambda_G}.$$
This finishes the proof of the Cheeger's inequality.


==> sections/warmup.tex <==
\section{Warm up: Cheeger's Inequality with a Buffer for \texorpdfstring{$k=2$}{k=2}}\label{sec:warm-up}

We now provide a self-contained proof of the upper bound in Theorem~\ref{thm:main} for $k=2$. While there are many new ideas needed to handle the setting for general $k$, this simpler setting already demonstrates how one can leverage buffers to obtain an improved upper bound. When $k=2$, we will consider cuts $(S,T)$ with a common buffer $B$. Such cuts consist of three disjoint sets $S$, $T$, and $B$ that partition the set of vertices $V$ into three groups. We will refer to such a partition as $(S,T\parallel B)$.
\iffalse
The $\varepsilon$-buffered edge expansion $G$ is defined as $$h_{G}^{2,\varepsilon} =
\min_{\substack{S, B: S\cap B = \varnothing;\\|S|\leq n/2;\; |B|\leq \varepsilon |S|}}
\left(\frac{|\delta(S, V \setminus (S \cup B))|}{|E|} \left/
\frac{|S|}{|V|}\right. \right).$$
In this definition, the size of the buffer $B$ is at most $\varepsilon |S|$.
\fi
\begin{proposition}\label{prop:cheeger}
Let $\varepsilon \in (0,1/4)$.
Consider any $d$-regular graph $G=(V,E)$ and let $\lambda_G$ be the second smallest eigenvalue of $L_G$, the normalized Laplacian of $G$. Then in polynomial time we can find three disjoint sets $\hat{S}, \hat{B}, \hat{T} $ with $\hat{S}\cup \hat{B}\cup \hat{T} = V$, $|\hat{S}| \le n/2$ and $|\hat{B}| \le 4\varepsilon \min(|\hat{S}|,|\hat{T}|)$ such that  
$$%h_G^{2,\varepsilon} \leq 
\phi_G(\hat{S},\hat{T}\parallel \hat{B}) = \max\left(\frac{|\delta(\hat{S},\hat{T})|}{d |\hat{S}|}, \frac{|\delta(\hat{S},\hat{T})|}{d |\hat{T}|}\right)   \leq 4\Big(1+\frac{2}{\varepsilon}\Big)\lambda_G.
$$
$(\hat{S},\hat{T}\parallel \hat{B})$ is a $(4\varepsilon)$-buffered partition with buffered expansion at most $4\Big(1+\frac{2}{\varepsilon}\Big)\lambda_G$. 
\end{proposition}
% \begin{question}
% Can we obtain a lower bound on $h_G(\varepsilon)$?
% \end{question}

%The algorithm is similar to the standard algorithm based on thresholding 
\begin{proof} The proof follows the same general strategy as the standard proof of the Cheeger inequality. %, the algorithm thresholds the second eigenvector. %The main difference is the  thresholds the second eigenvector.  
%We will use almost the same algorithm for finding $S$, $T$, and $B$ as in the previous section. 
%We now prove the ``hard'' part of the inequality: $h_G^2/8\leq \lambda_G$. 
We show how to find a distribution over (buffered) partitions $(S, B, T)$ in the graph $G$, by thresholding the second eigenvector of $L_G$, such that:
$$
\text{(I) } \E|\delta(S,T)| \leq (1+1/\varepsilon)\lambda_G\cdot d \E|S|\quad\text{ and }\quad
\text{(II) } \E|B| \le \varepsilon \E|S|.$$ 

\noindent 
The first condition gives an upper bound on the expected number of (non-buffered) edges crossing the cut, while the second condition gives a bound on the expected size of the buffer.  A simple probabilistic argument (see Lemma~\ref{lem:both-hold}) allows us to conclude that there exists a single buffered threshold cut that simultaneously satisfies both the properties (with some slack). 



% Note that for every distribution of sets $S$ of size at most $n/2$, we have (prove it!) 
% $$h_G \leq \frac{\E|\delta(S,V\setminus S)|}{|E|} \left/
% \frac{\E|S|}{|V|} = \frac{\E|\delta(S,V\setminus S)|}{\E|S|} \cdot \frac{|V|}{|E|}\right.
% = \frac{2}{d}\cdot \frac{\E|\delta(S,V\setminus S)|}{\E|S|}.
% $$

Let $v$ be an eigenvector
of $L_G$ corresponding to $\lambda_G = \lambda_2$. Then, we have $v \perp \ONE$, %, in other words $v(1)+v(2)+\dots+v(n)=0$ 
and
\begin{equation}\label{eq:v-LG-v-bound}
\langle v, L_G v\rangle = \lambda_G \|v\|^2.    
\end{equation} 



\paragraph{Step 1. Splitting the vector.} 
For technical reasons, we need to split vector $v$ into two vectors $v_+$ and $v_-$ each having at most $n/2$ non-zero coordinates. %We do this as follows. 
We do this by following a standard trick that is often used in the proof of Cheeger's inequality. 
%We first sort the vertices of the graph in decreasing order of coordinate $v(i)$ i.e. we assume that $v(1)\geq v(2) \geq \dots \geq v(n)$. 

Let $z$ denote the $\lceil n/2 \rceil$-th largest coordinate in the vector $v$. Then 
%Denote $m=\roundup{n/2}$; and the median value $\mu = v(m)$, and 
we shift the entire vector $v$ by $z$ and get $v' = v - z\ONE$. 
Since $v \perp \ONE$, the value of $\langle v', L_G v' \rangle/ \|v'\|^2$ is at most $\lambda_G$.  
%First, we sort the vertices of the graph in decreasing order i.e. we assume that $v(1)\geq v(2) \geq \dots \geq v(n)$. Denote $m=\roundup{n/2}$; and
%$\mu = v(m)$. Then, $\mu$ is the median of $v(1),\cdots, v(n)$. 
We now split the vector $v'$ into two vectors $v_+, v_-$ with disjoint supports as follows:
$$v_+ (i)= \begin{cases}
v(i) - z,& \text{if } v(i) \geq z;\\
0,& \text{otherwise},
\end{cases} \qquad
 v_- (i)= \begin{cases}
0,& \text{if } v(i) \geq z;\\
v(i)- z,& \text{otherwise}.
\end{cases}
$$

We show that there exists a vector $u \in \{v_+, v_- \}$ such that $\langle u, L_G u \rangle/ \|u\|^2$ is at most $\lambda_G$. See Claim~\ref{cl:v-plus-v-minus} in Appendix~\ref{app:cheeger} for a detailed proof. Next, we show that there exists an $\varepsilon$-buffered partition with small expansion by thresholding on this vector $u$. 

% \noindent A standard argument shows that we can proceed with at least one of the vectors $v_+$ or $v_-$ (see Claim~\ref{cl:v-plus-v-minus} in Appendix~\ref{app:cheeger}): 
% \begin{equation*}
% \exists u \in \{v_+, v_- \} \text{ s.t. }   \langle u, L_G u\rangle \leq \lambda_G \|u\|^2.
% \end{equation*}

For simplicity, we assume without loss of generality that $\|u\|_\infty =1$ (otherwise we can scale $u$ appropriately). 
% We will show that at least one of the following inequalities holds: $\langle v_+, L_G v_+\rangle \leq \lambda_G \|v_{+}\|^2$ or $\langle v_-, L_G v_-\rangle \leq \lambda_G \|v_{-}\|^2$. These inequalities are similar to the bound (\ref{eq:v-LG-v-bound}) we have for vector $v$. 

% \begin{claim}\label{cl:v-plus-v-minus}
% For vectors $v_+$ and $v_-$ defined above, we have 
% \begin{enumerate}
%     \item $\|v\|^2  \leq \|v_{+}\|^2 + \|v_{-}\|^2;$ and
%     \item $\langle v, L_G v\rangle \geq\langle v_+, L_G v_+\rangle +  \langle v_-, L_G v_-\rangle$;
%     \item $\langle v_+, L_G v_+\rangle \leq \lambda_G \|v_{+}\|^2$ or $\langle v_-, L_G v_-\rangle \leq \lambda_G \|v_{-}\|^2$.
% \end{enumerate}
% \end{claim}


\paragraph{Step 2. Random Thresholding with Buffers.}

We pick a random threshold $t \in [0,1]$  uniformly distributed in $[0,1]$ and define sets $S$, $T$ and buffer $B$ as follows:
\begin{align}\label{eq:cheeger2:defs}
  S&=\{i: u(i)^2 > t\}\\ T&=\big\{i: u(i)^2 \leq \sfrac{t}{(1+\varepsilon)}\big\}, \\
   B&= V \setminus (S\cup T) = 
\big\{i: \sfrac{t}{(1+\varepsilon)} < u(i)^2 \le t \big\}. 
\end{align}
% We define $S$ in exactly the same way as before:
% $$S=\{i: u(i)^2 > t\}.$$
% Similarly, define $T$ as
% $$T=\{i: u(i)^2 \leq t/(1+\varepsilon)\}.$$
% Then, the buffer $B$ between $S$ and $T$ equals 
% $$B= V \setminus (S\cup T) = 
% \{i: u(i)^2 \in[t/(1+\varepsilon), t)\}.
% $$
Note that $B \cup S= \{i: u(i)^2  > \sfrac{t}{(1+\varepsilon)}\}$. Since $t$ is picked uniformly from $[0,1]$ and $\|u\|_\infty =1$, we have $\E|S|= \sum_{i=1}^n \Pr\{i\in S\} = \sum_{i=1}^n u(i)^2 = \|u\|^2$, and
\begin{align}
    \E|B\cup S| &= \sum_{i=1}^n \min((1+\varepsilon)|u(i)|^2,1) \leq (1+\varepsilon)\|u\|^2. 
\end{align}
Thus,
$\E|B| \leq \varepsilon \|u\|^2 = \varepsilon \E|S|$, as stated in  Equation~(II).
Since $u(i) = 0$ for at least $\lceil n/2\rceil$ values of $i$ by our choice of $z$, $u(i) > t$ for at most $\lceil n/2\rceil$ values of $i$. Hence, $|S|\leq n/2$.

Note that for every edge $(i,j)$ from $S$ to $T$, we have $u(i)^2 > t > t/(1+\varepsilon) \geq u(j)^2$. Thus, for all edges $(i,j) \in \delta(S,T)$, we have: (a) $i\in S, j\in T$ if $u(i)^2 > u(j)^2$ and (b) $i\in T, j\in S$ if $u(i)^2 < u(j)^2$. 
%For convenience, assume that  every edge $(i,j)\in E$ is directed from $i$ to $j$ such that $u(i)^2 > u(j)^2$. Then, an edge $(i,j)$ belongs to $\delta(S,T)$ if and only if $i\in S$ and $j\in T$. 
Now consider an edge $(i,j) \in E$ with $u(i)^2 > u(j)^2$.
The probability that $(i,j)\in \delta(S,T)$  equals
\begin{align*}
\Pr\{(i,j)\in \delta(S,T)\}&=
\Pr\{i\in S; j\in T\} = 
\Pr\{t \leq u(i)^2\;\;\&\;\; t \geq (1 + \varepsilon) u(j)^2\}\\
&= \max\{u(i)^2 - (1 + \varepsilon) u(j)^2, 0\}.
\end{align*}
To bound the right side, we use the following simple claim.
\begin{claim}\label{cl:a-minus-b}
For all $\varepsilon>0$ and all real numbers $a$ and $b$, we have
$$a^2 - (1+\varepsilon) b^2 \leq (1+\nicefrac{1}{\varepsilon}) (a-b)^2.$$
\end{claim}
\begin{proof}
 If $b=0$, then the inequality holds. Assume, that $b\neq 0$. Divide both sides by $b^2$ and denote $\lambda = a/b$. We need to show that
$(1+\nicefrac{1}{\varepsilon})(\lambda-1)^2
 - \big(\lambda^2 -(1+\varepsilon)\big) \geq 0$.
 Write,
 \begin{align*}
 (1+\nicefrac{1}{\varepsilon})(\lambda-1)^2
 - \big(\lambda^2 -(1+\varepsilon)\big) &= 
 \nicefrac{1}{\varepsilon} \lambda^2 - 2(1+\nicefrac{1}{\varepsilon})\lambda + (\sqrt{\varepsilon} + \nicefrac{1}{\sqrt{\varepsilon}})^2\\
 &= (\nicefrac{\lambda}{\sqrt{\varepsilon}} - (\sqrt{\varepsilon} + \nicefrac{1}{\sqrt{\varepsilon}}))^2 \geq 0.\qedhere
 \end{align*}
\end{proof}

\noindent Hence from the above Claim~\ref{cl:a-minus-b}, we have
%$$\Pr\{i\in S; j\in T\} \leq (1+\nicefrac{1}{\varepsilon})(u(i) - u(j))^2.$$
%Hence, 
$$
\Pr\{i\in S; j\in T\} \leq (1+\nicefrac{1}{\varepsilon})(u(i) - u(j))^2.$$
By linearity of expectation, 
\begin{multline*}
\E|\delta(S,T)| \leq (1+\nicefrac{1}{\varepsilon})
\sum_{\substack{(i,j)\in E\\u(i)^2 > u(j)^2}} (u(i) - u(j))^2 \stackrel{\text{\tiny by (\ref{eq:lapl})}}{=} 
d (1+\nicefrac{1}{\varepsilon}) \langle u, L_G u\rangle \leq \\
\leq d (1+\nicefrac{1}{\varepsilon})\lambda_G \|u\|^2\leq d(1+\nicefrac{1}{\varepsilon})\lambda_G \cdot \E|S|.
\end{multline*}
Thus, this distribution over buffered partitions $(S,T \parallel B)$ 
%by thresholding on the vector $u$ 
satisfies Equation (I).
Since (I) and (II) both hold, we can use Lemma~\ref{lem:both-hold} (see below) to conclude that there exists a cut $(\hat S,\hat T)$ with buffer $\hat B$ for which 
$$ 
|\delta(\hat S,\hat T)| \leq 2d(1+\nicefrac{1}{\varepsilon})\lambda_G |\hat S|\text{ and }
|\hat B| \leq  2\varepsilon|\hat{S}|.
$$
For this cut $(\hat S,\hat T)$ with buffer $\hat B$, we have
$$ 
\frac{|\delta(\hat S,\hat T)|}{d|\hat S|} \leq \frac{2d(1+\nicefrac{1}{\varepsilon})\lambda_G |\hat S|}{d |\hat S|} = 2d(1+\nicefrac{1}{\varepsilon})\lambda_G.
$$
Since $|\hat{T}|/|\hat{S}| = (n - |\hat{S}| - |\hat{B}|)/|\hat{S}| \geq (2 - 1 - 2\varepsilon) = 1 -2\varepsilon$, we have
\begin{align*} 
\frac{|\delta(\hat S,\hat T)|}{d|\hat T|} &\leq \frac{2}{1 -2\varepsilon}d(1+\nicefrac{1}{\varepsilon})\lambda_G \leq 
4d(1+\nicefrac{1}{\varepsilon})\lambda_G\\
|\hat{B}| &\leq 2\varepsilon |\hat{S}|\leq \frac{2\varepsilon}{1-2\varepsilon} |\hat{T}|\leq 4\varepsilon |\hat{T}|.
\end{align*}
%
To finish the proof, it remains to show Lemma~\ref{lem:both-hold}.

\end{proof}
\begin{lemma}\label{lem:both-hold}
Consider arbitrary jointly distributed non-negative random variables $X$, $Y$, $Z$. Suppose that $\E[X] \leq \alpha \E[Z]$ and $\E[Y] \leq \beta \E[Z]$. Then,
\begin{equation}\label{eq:pr-both-hold}
\Pr\{X \le 2\alpha Z \text{ and }Y \leq 2\beta Z\} > 0.  \end{equation}
\end{lemma}
\begin{proof}
Consider random variables $X/(2\alpha) + Y/(2\beta)$. We have $\E[Z] \geq \E[X/(2\alpha) + Y/(2\beta)]$. This implies that $\Pr\{Z \geq X/(2\alpha) + Y/(2\beta)]\}> 0$; otherwise we would have $\E[Z - X/(2\alpha) - Y/(2\beta)]<0$. 
However, if $Z \geq X/(2\alpha) + Y/(2\beta)$, then 
$X \leq 2\alpha Z$ and $Y \leq 2\beta Y$. Therefore,
inequality (\ref{eq:pr-both-hold}) holds.
\end{proof}


